A Parameter-efficient Language Extension Framework for Multilingual ASR

Covering all languages with a multilingual speech recognition model (MASR) is very difficult. Performing language extension on top of an existing MASR is a desirable choice. In this study, the MASR continual learning problem is probabilistically decomposed into language identity prediction (LP) and cross-lingual adaptation (XLA) sub-problems. Based on this, we propose an architecture-based framework for language extension that can fundamentally solve catastrophic forgetting, debudded as PELE. PELE is designed to be parameter-efficient, incrementally incorporating an add-on module to adapt to a new language. Specifically, different parameter-efficient fine-tuning (PEFT) modules and their variants are explored as potential candidates to perform XLA. Experiments are carried out on 5 new languages with a wide range of low-resourced data sizes. The best-performing PEFT candidate can achieve satisfactory performance across all languages and demonstrates superiority in three of five languages over the continual joint learning setting. Notably, PEFT methods focusing on weight parameters or input features are revealed to be limited in performance, showing significantly inferior extension capabilities compared to inserting a lightweight module in between layers such as an Adapter.

==> peft.tex <==
Low-rank adaptation (LoRA) \cite{DBLP:conf/iclr/HuSWALWWC22} is the most representative PEFT method to make incremental updates to weight matrices. It assumes the desired weight update can be decomposed into two small low-rank weight matrices, thus largely reducing the required trainable parameters. For a weight matrix $\mathbf{W}_0 \in \mathbb{R}^{d_2 \times d_1}$, the incremental update $\Delta \mathbf{W} = \mathbf{B}\mathbf{A}$, where $\mathbf{B} \in \mathbb{R}^{d_2 \times r}$, $\mathbf{A} \in \mathbb{R}^{r \times d_1}$ and the rank $r \ll min(d_1, d_2)$. To increase the adaptation capacity of the vanilla LoRA, we propose the improved LoRA variant as follows:
\begin{align}
    \label{eq:lora}
    \mathbf{W} = \mathbf{W}_0 \odot \mathbf{W}_s + \Delta \mathbf{W}, \\
    \mathbf{W}_s = \mathbf{B}\mathbf{S}_s\mathbf{A};~~ \Delta \mathbf{W} = \mathbf{B}\mathbf{S}_{\Delta}\mathbf{A},
\end{align}
where $\mathbf{W}_s \in \mathbb{R}^{d_2 \times d_1}$ is used to scale the original weight elementwisely and $\mathbf{\Delta W}$ is the incremental update as before. $\mathbf{S}_{\Delta} \in \mathbb{R}^{r \times r}$ is a diagonal matrix, including $r$ coefficients to control the importance of the corresponding rank of $\mathbf{B}$ and $\mathbf{A}$. With different diagonal matrix $\mathbf{S}_{s}  \in \mathbb{R}^{r \times r}$, $\mathbf{W}_s$ is similarly decomposed as $\Delta\mathbf{W}$ and share the same low-rank matrices.

Instead of directly adjusting the parameter weights, a recently popular method, mask tuning, opts to change the weight connection. It is achieved by multiplying the original weight matrix $\mathbf{W}_0$ with a binary mask $\mathbf{B} \in \{0,1\}^{d_2 \times d_1}$ as follows:
\begin{equation}
    \label{eq:mask}
    \mathbf{W} = \mathbf{W}_0 \odot \mathbf{B};~~  \mathbf{B} = \mathbbm{1}_{\mathbf{W}_{m} > r},
\end{equation}
where $\mathbbm{1}_{(.)}$ is an indicator function conditioned on the inequality $\mathbf{W}_{m} > r$. $\mathbf{W}_{m} \in \mathbb{R}^{d_2 \times d_1}$ is the learnable mask weight. $r$ is the mask threshold predefined or derived by a sparsity ratio. 

Mask tuning has shown promising results for adapting the pre-trained speech model XLSR to multiple languages \cite{fu2022losses, yu2023master}.  On extremely low-resource conditions (one-hour data), it has better performance than the traditional weight tuning, while being more generalized. We argue that the learning capacity of mask tuning is limited and may be proper to be combined with LoRA for meanwhile adjusting the weight on those unmasked connections. To this end, we propose MaskLoRA as follows:
\begin{equation}
    \label{eq:makslora}
    \mathbf{W} = (\mathbf{W}_0 \odot \mathbf{W}_s + \Delta \mathbf{W}) \odot \mathbf{B},
\end{equation}
where it directly combines the Eq. \ref{eq:lora} and Eq. \ref{eq:mask}.

\subsubsection{Function composition}
Adapter \cite{houlsby2019parameter} is a lightweight module that consists of a down-projection matrix $\mathbf{W}_d$ , ReLU activation, and up-projection matrix $\mathbf{W}_u$. It is often inserted in between layers and the adapter output $\mathbf{H}_{i}^{'}$ would replace the original input $\mathbf{H}_i$ to the next layer:
\begin{equation}
    \mathbf{H}_{i}^{'} = Adapter(\mathbf{H}_{i})  = (ReLU(\mathbf{H}_{i}\mathbf{W}_{d}))\mathbf{W}_{u},
\end{equation}



==> table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\centering
\caption{The WER (\%) performance comparison of MASR continual learning between baselines and the proposed PELE. $base10$ represents the average recognition performance on the original 10 languages that the base model is trained with. $Avg$ represents the averaged WER of all 16 languages. ER (1k) denotes 1k utterances per language are cached for experience replay. In the $\alpha$ column, $LP~post$ means $\alpha$ adopts the LID prediction posterior, while $LP~ohot$ denotes the one-hot vector derived by $LP~post$ is used. $GT~ohot$ means adopting the ground-truth one-hot vector and $GT~learn$ refer to the learnable vector parameters that initialized as $GT~ohot$.        }
\resizebox{1.04\linewidth}{!}{
\begin{tabular}{cc|cccccccc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inc. \\ Params\end{tabular}}} & \multirow{2}{*}{base10} & \multirow{2}{*}{de} & \multirow{2}{*}{pl} & \multirow{2}{*}{cy} & \multirow{2}{*}{ja} & \multicolumn{1}{c|}{\multirow{2}{*}{cs}} & \multirow{2}{*}{Avg} \\
\multicolumn{2}{c|}{}                         & \multicolumn{1}{c|}{}                                                                        &                         &                     &                     &                     &                     & \multicolumn{1}{c|}{}                    &                      \\ \midrule
\multicolumn{2}{c|}{Mono}                     & \multicolumn{1}{c|}{43.4}                                                                    & 21.1                    & 15.1                & 10.8                & 15.5                & 19.3                & \multicolumn{1}{c|}{83.8}                & 22.2                 \\
\multicolumn{2}{c|}{Raw}                      & \multicolumn{1}{c|}{0}                                                                       & 16.3                    & 90.8                & 104.0               & 99.7                & 104.2               & \multicolumn{1}{c|}{103.1}               & 41.6                 \\
\multicolumn{2}{c|}{FullFT}                   & \multicolumn{1}{c|}{186.5}                                                                   & 99.8                    & 12.8                & 8.0                 & 10.5                & 8.5                 & \multicolumn{1}{c|}{24.5}                & 66.4                 \\
\multicolumn{2}{c|}{ER (1k)}                  & \multicolumn{1}{c|}{0}                                                                       & 48.3                    & 14.9                & 11.6                & 13.3                & 10.5                & \multicolumn{1}{c|}{29.5}                & 35.1                 \\
\multicolumn{2}{c|}{ER (10k)}                 & \multicolumn{1}{c|}{0}                                                                       & 23.4                    & 15.2                & 14.0                & 14.2                & 11.1                & \multicolumn{1}{c|}{30.9}                & 20.0                 \\
\multicolumn{2}{c|}{CJT}                      & \multicolumn{1}{c|}{0}                                                                       & 14.8                    & 15.2                & 12.5                & 15.9                & 13.3                & \multicolumn{1}{c|}{32.0}                & 14.8                 \\ \midrule
$\alpha$                          & PEFT         &                                                                                              & \multicolumn{7}{c}{PELE framework}                                                                                                                                                \\ \midrule
LP post                        & Adapter      & \multicolumn{1}{c|}{11.2}                                                                    & 16.3                    & 23.0                & 24.4                & 17.1                & 15.1                & \multicolumn{1}{c|}{35.4}                & 17.4                 \\
LP ohot                        & Adapter      & \multicolumn{1}{c|}{11.2}                                                                    & 16.3                    & 24.1                & 27.9                & 16.9                & 14.6                & \multicolumn{1}{c|}{32.4}                & 17.4                 \\ \hline
\multirow{3}{*}{GT ohot}       & LoRA         & \multicolumn{1}{c|}{11.3}                                                                    & 16.3                    & 31.0                & 33.3                & 29.0                & 29.7                & \multicolumn{1}{c|}{49.2}                & 21.0                 \\
                               & LoRA*        & \multicolumn{1}{c|}{16.2}                                                                    & 16.3                    & 28.1                & 26.4                & 24.5                & 22.7                & \multicolumn{1}{c|}{43.1}                & 19.2                 \\
                               & Adapter      & \multicolumn{1}{c|}{11.2}                                                                    & 16.3                    & 19.6                & 14.2                & 13.9                & 12.7                & \multicolumn{1}{c|}{26.5}                & 15.6                 \\ \hline
GT learn                       & Adapter      & \multicolumn{1}{c|}{11.2}                                                                    & 16.3                    & 18.3                & 12.8                & 13.9                & 12.4                & \multicolumn{1}{c|}{29.9}                & 15.7                 \\ \bottomrule
\end{tabular}
\label{tab:res}
\end{table}

\begin{table*}[t!]
\centering
\caption{The WER (\%) performance comparison of MASR continual learning between baselines and the proposed PELE. $base10$ represents the average recognition performance on the original 10 languages that the base model is trained with. $Avg$ represents the averaged WER of all 16 languages. ER (1k) denotes 1k utterances per language are cached for experience replay. In the $\alpha$ column, $LP~post$ means $\alpha$ adopts the LID prediction posterior, while $LP~ohot$ denotes the one-hot vector derived by $LP~post$ is used. $GT~ohot$ means adopting the ground-truth one-hot vector and $GT~learn$ refer to the learnable vector parameters that initialized as $GT~ohot$.        }
\resizebox{0.78\linewidth}{!}{
\begin{tabular}{cc|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Methods}       & Inc. Params (M) & \multicolumn{1}{c|}{base10} & de   & pl    & cy   & ja    & \multicolumn{1}{c|}{cs}    & \multicolumn{1}{c|}{new5}  & Avg  \\ \midrule
\multicolumn{2}{c|}{Mono}          & 43.4       & \multicolumn{1}{c|}{21.1}   & 15.1 & 10.8  & 15.5 & 19.3  & \multicolumn{1}{c|}{83.8}  & \multicolumn{1}{c|}{28.9}  & 22.2 \\
\multicolumn{2}{c|}{Raw}           & 0          & \multicolumn{1}{c|}{16.3}   & 90.8 & 104.0 & 99.7 & 104.2 & \multicolumn{1}{c|}{103.1} & \multicolumn{1}{c|}{100.3} & 41.6 \\
\multicolumn{2}{c|}{FullFT}        & 186.5      & \multicolumn{1}{c|}{99.8}   & 12.8 & 8.0   & 10.5 & 8.5   & \multicolumn{1}{c|}{24.5}  & \multicolumn{1}{c|}{12.9}  & 66.4 \\
\multicolumn{2}{c|}{ER (1k)}       & 0          & \multicolumn{1}{c|}{48.3}   & 14.9 & 11.6  & 13.3 & 10.5  & \multicolumn{1}{c|}{29.5}  & \multicolumn{1}{c|}{15.9}  & 35.1 \\
\multicolumn{2}{c|}{ER (10k)}      & 0          & \multicolumn{1}{c|}{23.4}   & 15.2 & 14.0  & 14.2 & 11.1  & \multicolumn{1}{c|}{30.9}  & \multicolumn{1}{c|}{17.1}  & 20.0 \\
\multicolumn{2}{c|}{CJT}           & 0          & \multicolumn{1}{c|}{14.8}   & 15.2 & 12.5  & 15.9 & 13.3  & \multicolumn{1}{c|}{32.0}  & \multicolumn{1}{c|}{17.8}  & 14.8 \\ \midrule
$\alpha$                    & PEFT    &            & \multicolumn{8}{c}{PELE framework}                                                                                         \\ \midrule
LP post                  & Adapter & 11.2       & \multicolumn{1}{c|}{16.3}   & 23.0 & 24.4  & 17.1 & 15.1  & \multicolumn{1}{c|}{35.4}  & \multicolumn{1}{c|}{23.0}  & 17.4 \\
LP ohot                  & Adapter & 11.2       & \multicolumn{1}{c|}{16.3}   & 24.1 & 27.9  & 16.9 & 14.6  & \multicolumn{1}{c|}{32.4}  & \multicolumn{1}{c|}{23.2}  & 17.4 \\ \hline
\multirow{3}{*}{GT ohot} & LoRA    & 11.3       & \multicolumn{1}{c|}{16.3}   & 31.0 & 33.3  & 29.0 & 29.7  & \multicolumn{1}{c|}{49.2}  & \multicolumn{1}{c|}{34.4}  & 21.0 \\
                         & LoRA*   & 16.2       & \multicolumn{1}{c|}{16.3}   & 28.1 & 26.4  & 24.5 & 22.7  & \multicolumn{1}{c|}{43.1}  & \multicolumn{1}{c|}{28.9}  & 19.2 \\
                         & Adapter & 11.2       & \multicolumn{1}{c|}{16.3}   & 19.6 & 14.2  & 13.9 & 12.7  & \multicolumn{1}{c|}{\textbf{26.5}}  & \multicolumn{1}{c|}{\textbf{17.4}}  & \textbf{15.6} \\ \hline
GT learn                 & Adapter & 11.2       & \multicolumn{1}{c|}{16.3}   & \textbf{18.3} & \textbf{12.8}  & \textbf{13.9} & \textbf{12.4}  & \multicolumn{1}{c|}{29.9}  & \multicolumn{1}{c|}{17.5}  & 15.7 \\ \bottomrule
\end{tabular}}
\label{tab:res}
\end{table*}
